The Informational Role of Online Recommendations: Evidence from a Field Experiment

We conduct a field experiment on a movie-recommendation platform to investigate whether and how online recommendations influence consumption choices. Using a within-subjects design, our experiment measures the causal effect of recommendations on consumption and decomposes the relative importance of two economic mechanisms: expanding consumers' consideration sets and providing information about their idiosyncratic match value. We find that the informational component exerts a stronger influence - recommendations shape consumer beliefs, which in turn drive consumption, particularly among less experienced consumers. Our findings and experimental design provide valuable insights for the economic evaluation and optimisation of online recommendation systems.

==> Tables/table-iv-consumption-on-beliefs-1st-elicit.tex <==
\begin{tabular}{l@{\extracolsep{4pt}}ccc@{}}
  \hline\hline
  & \multicolumn{3}{c}{Consumption} \\
  \cline{2-4}
  \hspace*{9em} & (1) & (2) & (3) \\
  \hline
  Uncertainty & $-$0.159$^{**}$ &  & $-$0.162$^{**}$ \\ 
  & (0.067) &  & (0.075) \\ [.1em]
  Exp. Match Value &  & 0.062$^{***}$ & 0.091$^{**}$ \\ 
  &  & (0.019) & (0.037) \\ [.1em]
  Constant & 0.558$^{**}$ & $-$0.171$^{***}$ & 0.293 \\ 
  & (0.229) & (0.057) & (0.226) \\ [.1em]
  \hline \\
  Observations & 20,895 & 20,895 & 20,895 \\ 
  \hline\hline
  \multicolumn{4}{l}{\footnotesize Clustered standard errors at the subject level in parentheses.}\\
  \multicolumn{4}{l}{\footnotesize $^{*}$ \(p<0.1\), $^{**}$ \(p<0.05\), $^{***}$ \(p<0.01\)}
\end{tabular}

==> Tables/table-iv-consumption-on-beliefs.tex <==
\begin{tabular}{l@{\extracolsep{4pt}}ccc@{}}
  \hline\hline
  \hspace*{9em} & \multicolumn{3}{c}{Consumption} \\
  \cline{2-4}
  \hspace*{9em} & (1) & (2) & (3) \\
  \hline
  Uncertainty & $-$0.139$^{***}$ &  & $-$0.126$^{**}$ \\ 
   & (0.054) &  & (0.054) \\ [.1em]
  Exp. Match Value &  & 0.061$^{***}$ & 0.082$^{***}$ \\ 
   &  & (0.019) & (0.029) \\ [.1em]
  Constant & 0.486$^{***}$ & $-$0.168$^{***}$ & 0.195 \\ 
   & (0.181) & (0.056) & (0.172) \\ [.1em]
  \hline \\
  Observations & 20,895 & 20,895 & 20,895 \\ 
  \hline\hline
  \multicolumn{4}{l}{\footnotesize Clustered standard errors at the subject level in parentheses.}\\
  \multicolumn{4}{l}{\footnotesize $^{*}$ \(p<0.1\), $^{**}$ \(p<0.05\), $^{***}$ \(p<0.01\)}
\end{tabular}

==> preamblepaper.tex <==
%%% Fonts & Symbols %%%
%LaTeX
\usepackage[utf8]{inputenc} 													% Special characters; LaTeX
\usepackage[T1]{fontenc} 														% Special characters; LaTeX
% \fontfamily{lmodern}															% Font; default LaTeX font; LaTeX
%\usepackage[letterspace=0]{microtype} 							 				% Shrink spacing between letters; doesn't work with XeLaTeX
%	\SetTracking{encoding=*}{-500}												%\textls[-100]{shrink space between letters}

%Both LaTeX and XeLaTeX
\usepackage{soul}							 										% Highlighting text (did NOT test with XeLaTex)
\usepackage[portuguese, english]{babel} 										% Language package for special characters
\usepackage{cjhebrew}
\usepackage[space, extendedchars, multidot]{grffile} 							% Special characters
\usepackage[official]{eurosym} 													% Euro symbol
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor} 						% Font colours; simply use e.g. {\color{red} some text} to colour font; cannot be used with Beamer

%%% Format Paragraph %%%
\usepackage{ragged2e} 															% Enables justifying text using {\justify text}
\usepackage{setspace} 															% Setspace respects body, footnotes and captions spacing
\usepackage{multicol} 															% Multicolumn in text
\usepackage[flushmargin,bottom]{footmisc}									% Enables formatting footnotes
%\usepackage{dblfnote} 															% Double column in footnotes
\usepackage[all]{nowidow}														% Prevent isolated words at the end of the page
\setlength{\columnsep}{0.5cm} 													% Set the gap between the columns
\interfootnotelinepenalty=10000 												% Prevents breaking footnotes across pages
\setlength{\parskip}{0.5em} 													% Paragraph Spacing
\setlength{\parindent}{0.25cm} 													% Paragraph Indenting;
%!!USES setspace PACKAGE
%\singlespacing 																% Line Single Spacing
%\onehalfspacing 																% Line 1.5 Spacing
%\doublespacing 																% Line 2.0 Spacing
\setstretch{1} 																	% Line 1.25 Spacing
%\begin{doublespace}\end{doublespace} 											% Specific doublespace environment
%\begin{spacing}{2.5}\end{spacing} 												% Specific customized line spacing environment
%{\addfontfeatures{LetterSpace-6} write text here} 								% Shrink spacing between letters for a spefic part of the document; addfontfeatures serves to add all types of font features; used with fontspec
\setlength\footnotemargin{10pt} 												% Specific footnote margin
\raggedbottom																	% Prevents large blanks in the middle of the page													% Define counters (equations, footnotes, theorems, etc.)
%\counterwithout{footnote}{chapter}									% Prevent footnotes to restart from 1 at each chapter
%\counterwithout{figure}{chapter}										% Prevent figures to restart from 1 at each chapter
%\counterwithout{table}{chapter}											% Prevent tables to restart from 1 at each chapter
%\makeatletter
%        \@addtoreset{footnote}{part}    							% Reset footnote every part
%        \@addtoreset{figure}{part}    							% Reset footnote every part
%        \@addtoreset{table}{part}    							% Reset footnote every part
%\makeatother
%\renewcommand\thefigure{\arabic{part}.\arabic{figure}}				% Inserts the part number in the figure numbering
%\renewcommand\thetable{\arabic{part}.\arabic{table}}				% Inserts the part number in the table numbering
\usepackage{courier} 															% Code-like font
\usepackage{tocloft}															% Format TOC
\usepackage{pdfpages}														% Include pdf files keeping the header
\usepackage{lastpage}														% Set \pageref{LastPage} for last page counter
\usepackage{textcomp}

%%% Math %%%
%\usepackage{amsmath}															% Basic math characters; included in mathtools
\usepackage{amsfonts}															% Fonts from the American Mathematical Society
\usepackage{amsthm}												  				% Theorem package
\usepackage{thmtools}												  				% Theorem package; allows to define styles
\usepackage{mathtools}															% Basic math characters
\usepackage{amsbsy} 															% Bold symbols with \pmb
\usepackage{amssymb}															% Basic math symbols
\usepackage{bbm}																% Blackboard-style math characters
\usepackage{units}																% Nice diagonal fractions
%\usepackage{bm}																% Bold sym­bols in maths mode; Conflicts with XeLaTeX
\usepackage{bbm}																% Indicator function
\usepackage{empheq} 															% Emphasize equations
\usepackage{centernot} 															% "Not" can be applied to any symbol; does not work with XeLaTeX
\usepackage{tensor}			 													% Enables ordering of superscripts and subscripts
%\usepackage{mathspec}															% Specify arbitrary fonts for mathematics; Use only with XeLaTeX; Conflicts with amsmath
\usepackage{txfontsb}		 													% Enables usage of varmathbb
\usepackage{relsize,exscale}
%%% Math: Format Space around enviroments %%%
%\makeatletter
%\g@addto@macro\normalsize{%
%  \setlength\abovedisplayskip{10pt}
%  \setlength\belowdisplayskip{10pt}
%  \setlength\abovedisplayshortskip{10pt}
%  \setlength\belowdisplayshortskip{10pt}
%}
%\makeatother


%%% Math Commands %%%
\newcommand*\widefbox[1]{\fbox{\hspace{2em}#1\hspace{2em}}}						% Emphasize equations use comand \widefbox
% \newcommand{\C}{{\varmathbb{C}}}										% Defines command \C to denote Complex
% \newcommand{\R}{{\varmathbb R}} 													% Defines command \R to denote Reals
% \newcommand{\Q}{{\varmathbb{Q}}} 										% Defines command \Q to denote Rationals
% \newcommand{\Z}{{\varmathbb{Z}}}										% Defines command \Z to denote Integers
% \newcommand{\N}{{\varmathbb N}} 													% Defines command \N to denote Naturals
% \newcommand{\pd}{\partial} 														% Defines command \pd to denote partial derivatives
% \newcommand{\bimpl}{{\,\Leftrightarrow\,}} 										% Defines command \bimpl to denote long left-right arrow (bidirectional implication)
% \newcommand{\nbimpl}{{\,\nLeftrightarrow\,}} 										% Defines command \nbimpl to denote crossed long left-right arrow  (not bidirectional implication)
% \newcommand{\impl}{{\,\Rightarrow\,}} 										% Defines command \impl to denote long right arrow (implies)
% \newcommand{\nimpl}{{\,\nRightarrow\,}} 										% Defines command \nimpl to denote crossed long right arrow (does not imply)
% \newcommand{\limpl}{{\,\Leftarrow\,}} 										% Defines command \limpl to denote long left arrow (left-directional implication)
% \newcommand{\rar}{{\,\rightarrow\,}} 										% Defines command \rar to denote right arrow
% \newcommand{\nrar}{{\,\nrightarrow\,}} 										% Defines command \nrar to denote crossed right arrow
% \newcommand{\lar}{{\,\leftarrow\,}} 										% Defines command \lar to denote left arrow
% \newcommand{\nlar}{{\,\nleftarrow\,}} 										% Defines command \nlar to denote crossed left arrow
% \newcommand{\uar}{{\,\uparrow\,}} 										% Defines command \uar to denote up arrow
% \newcommand{\nuar}{{\,\nuparrow\,}} 										% Defines command \nuar to denote crossed up arrow
% \newcommand{\dar}{{\,\downarrow\,}} 										% Defines command \dar to denote down arrow
% \newcommand{\ndar}{{\,\ndownarrow\,}} 										% Defines command \ndar to denote crossed down arrow
% \newcommand{\lagr}{\mathcal{L}} 												% Defines command \lagr to denote the Lagrangian L
% \newcommand{\hami}{\mathcal{H}} 												% Defines command \hami to denote the Hamiltonian H
% \newcommand{\inc}{\Delta\,} 														% Defines command \inc to denote Delta for increment/variation symbol
% \newcommand{\ce}{\varepsilon} 														% Defines command \ce to denote curly epsilon
% \newcommand{\cphi}{\varphi} 														% Defines command \cphi to denote curly phi
% \newcommand{\bcs}{\backslash} 														% Defines command \bcs to denote backslash in math environment
% \newcommand{\ints}{\,\mathrm{int}\,}													% Defines command \ints to denote int [interior points of a set] in math environment
% \newcommand{\thf}{\,\therefore\,}													% Defines command \thf to denote \therefore in math environment
% \newcommand{\bec}{\,\because\,}													% Defines command \bec to denote \because in math environment
% \newcommand{\E}{\mathbb{E}}													% Defines command \E to denote E() in math environment
% \newcommand{\Var}{\mathbb{V}}													% Defines command \Var to denote Var() in math environment
% \newcommand{\Covar}{\text{Cov}}													% Defines command \Covar to denote Covar() in math environment
% \newcommand{\supp}{\text{supp}}													% Defines command \supp to denote Var() in math environment
% \newcommand{\pr}{\mathbb{P}}													% Defines command \var to denote P() in math environment
% \newcommand{\convp}{\overset{p}{\to}}								% Defines command \convp to denote convergence in probability in math environment
% \newcommand{\convd}{\overset{d}{\to}}								% Defines command \convp to denote convergence in distribution in math environment
% \newcommand{\indeprv}{\protect\mathpalette{\protect\independenT}{\perp}}								% Defines command \indeprv to denote independent random variables in math environment
% \def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
% \newcommand{\oset}{\varnothing} 														% Defines command \oset to denote empty set
\newcommand{\lrp}[1]{\left({#1}\right)}													% Defines command \lrp to denote left-right parenthesis
\newcommand{\lrb}[1]{\left\{{#1}\right\}}													% Defines command \lrb to denote left-right brackets
\newcommand{\lrsb}[1]{\left[{#1}\right]}													% Defines command \lrb to denote left-right brackets
% \newcommand{\indic}{\mathbbm{1}}													% Defines command \indic to denote indicator function
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\newcommand{\eqnumber}{\refstepcounter{equation}\tag{\theequation}} % Inserts number in equation within nonnumber environment
% \newcommand{\dis}{\displaystyle}										 % Renders inline equations as full display

%%% Math Theorems, Propositions and etc. %%%
		%\newtheorem{<name>}{<heading>}[<counter>]
					%will create an environment <name> for a theorem-like structure; the counter for this structure will be subordinated to <counter>. On the other hand, using
		%\newtheorem{<name>}[<counter>]{<heading>}
					%will create an environment <name> for a theorem-like structure; the counter for this structure will share the previously defined <counter> counter.
\theoremstyle{definition}
\newtheorem{thm}{Theorem} 												% Defines the theorem environment
\newtheorem{prop}{Proposition} 											% Defines the proposition environment
\newtheorem{corol}{Corollary} 											% Defines the corollary environment
\newtheorem{claim}{Claim} 												% Defines the corollary environment
\newtheorem{lemma}{Lemma} 												% Defines the lemma environment
\newtheorem{remark}{Remark} 											% Defines the remark environment
\newtheorem{hyp}{Hypothesis}											% Defines the hyp environment
\newtheorem{exmpl}{Example}												% Defines the exmpl environment
\newtheorem{dfn}{Definition}											% Defines the dfn environment
\newtheorem{assumption}{Assumption}	    								% Defines the assumption environment
\newtheorem{condition}{Condition}	    								% Defines the condition environment
\newtheorem{fact}{Fact}	            	    							% Defines the fact environment
\newtheorem{observ}{Observation}    	    							% Defines the fact environment
\newcommand*{\dfnend}{\hfill \rule{1.5pt}{1em}\,\rule{1.5pt}{1em}}
%\renewcommand\theprop{\arabic{part}.\arabic{prop}}				        % Inserts the part number in the proposition numbering
%\renewcommand\thetheorem{\arabic{part}.\arabic{theorem}}	    	    % Inserts the part number in the theorem numbering
%\renewcommand\thelemma{\arabic{part}.\arabic{lemma}}	    		    % Inserts the part number in the lemma numbering
%\renewcommand\theremark{\arabic{part}.\arabic{remark}} 			    % Inserts the part number in the remark numbering

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%%% Widebar %%%
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


%%% Graphics and Tables %%%
\usepackage{graphicx}															% Support for graphics
\usepackage{tabularx}															% Support for tables
\usepackage{ltablex}															% Long tables X
\usepackage{pdflscape}															% Landscape page contents
\usepackage{longtable} 															% Long tables
\usepackage{tabu} 																% Long tables with longtabu; define paragraphs; flexible tables
\usepackage{hhline} 															% Double hline in tables
\usepackage{booktabs} 															% Format tables; \toprule, \midrule, \bottomrule; informative and practical readme
\usepackage{multirow} 															% Multirow in tables
\usepackage[textfont=bf,hypcap]{caption}		 								% Format captions \label{sec:section} section label~\ref{sec:section}
\captionsetup{labelformat=simple,labelsep=period}						% Format table captions
%\usepackage[labelformat=empty]{caption} 										% Format captions
\usepackage{ragged2e}															% Align with \flushleft, etc
\usepackage{array}																% Matricial support
\usepackage{epstopdf}															% Include .eps graphics; does not work well with XeLaTeX
\usepackage{fancyref}															% Labeling details
%\usepackage{tikz-qtree} 														% Draw game theory extensive form graphs/trees
%\usepackage{stata}																% Import tables using sjlog, texdoc
\usepackage{fancyref}															% Details labeling
\usepackage{float}																% Prevent floats from floating
%\usepackage[capposition=top]{floatrow}					% Note for figures using \floatfoot{content...}
\newcommand\fignote[1]{\captionsetup{textfont=normal,font=small}\caption*{#1}}
\usepackage{pgfplots}
\pgfplotsset{compat=1.17}
\usetikzlibrary{calc}
\newcommand\payoff[1]{ $\begin{pmatrix} #1 \end{pmatrix}$} % Command for payoffs in game trees
\usepackage{dcolumn}
\usepackage{subcaption}

%%% Lists %%%
%\usepackage[ampersand]{easylist}												% List package
\usepackage{enumitem}															% Great list package
									% \begin{enumerate}[label=\roman*] or [label=\alph*] [label=\arabic*] or \Roman* or \Alph* or label=-, \bullet, or any other sign
									% To use embeded lists, use \begin{enumerate}[label=\arabic*.] for the first and \begin{enumerate}[label=\theenumi.(\roman*).] to get 1.i.
									% Anything can be used as a label, namely \bullet, \rhd, \circ, \Box, \rightarrow, \triangleright, \RIGHTarrow - see http://www.rpi.edu/dept/arc/training/latex/LaTeX_symbols.pdf for more symbols
									% It suffices to use \item to get the list
									% [...,noitemsep] kills the space between paragraphs within the list; nosep kills all vertical spacing
									% Resume keeps going at previous list
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$} % To-do lists
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}%
\hspace{-2.5pt}}
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}}


%%% Varia %%%
\usepackage{etoolbox}															% Extends TeX code
\usepackage{ifthen} 															% Produce if clauses
% \usepackage{datetime2} 															% Get month and time
% \makeatletter
% \newcommand*{\monthyeardate}{%
%   \DTMenglishmonthname{\@dtm@month}, \@dtm@year
% }
% \makeatother
% \makeatletter
% \newcommand*{\todaydate}{%
%   \DTMenglishmonthname{\@dtm@month} \@dtm@day, \@dtm@year
% }
% \makeatother
\usepackage{datetime} 															% Get month and time
% \usepackage{datetime2} 															% Get month and time

\newdateformat{MonthDDYYYY}{%
  \monthname[\THEMONTH] \THEDAY, \THEYEAR
  }
\newdateformat{MonthYYYY}{%
  \monthname[\THEMONTH] \THEYEAR
  }


%%% Format Headers/Footers and Chapters/Sections/Subsections/Subsubsections %%%%
\usepackage[sf,sl,outermarks]{titlesec}
\usepackage{titleps}
\setcounter{secnumdepth}{4}														% Depth in Table of Contents
\setcounter{tocdepth}{1}

\renewcommand*{\thepart}{}
\renewcommand*{\thechapter}{}
\renewcommand*{\thesection}{\arabic{section}.}
\renewcommand*{\thesubsection}{\thesection\,\arabic{subsection}.}
\renewcommand*{\thesubsubsection}{\thesubsection\,\arabic{subsubsection}}%\arabic{subsubsection}.}
%\numberwithin{equation}{section}
\renewcommand*{\theequation}{\arabic{equation}}
\titleclass{\part}{straight}
\titleclass{\chapter}{straight}


\titleformat{\part}[block]
  {\normalfont\Large\itshape\centering}{}{18pt}{\Large\bfseries}
\titlespacing*{\part}{0pt}{*1.5}{*0}											% Spacing before and after

\titleformat{\chapter}[block]
  {\normalfont\Large\bfseries\centering}{}{14pt}{\Large\bfseries}
\titlespacing*{\chapter}{0pt}{*1.5}{*2}											% Spacing before and after

\titleformat{\section}[block]													% Block to format
{\normalfont\Large\bfseries}{\thesection}{12pt}{\Large\bfseries}		% Formating the block
\titlespacing*{\section}{0pt}{*1.5}{*0}											% Spacing before and after

\titleformat{\subsection}[block]
{\normalfont\large\bfseries}{\thesubsection}{12pt}{\large\bfseries}
\titlespacing*{\subsection}{0pt}{*1}{*0.8}

\titleformat{\subsubsection}[block]
{\normalfont\large\itshape}{\thesubsubsection}{11pt}{\large\itshape}
\titlespacing*{\subsubsection}{0pt}{*1}{*0.8}

\titleformat{\paragraph}[block]
{\normalfont\normalsize\bfseries}{\hspace{-1cm}}{11pt}{\bfseries\normalsize}
\titlespacing*{\paragraph}{0pt}{*0.5}{*0.2}


%\makeatletter
%\patchcmd{\chapter}{\if@openright\cleardoublepage\else\clearpage\fi}{}{}{}
%\makeatother

%\makeatletter
%\@addtoreset{chapter}{part}										 % Reset chapter numbers for each part
%\makeatother

\renewcommand\cfttoctitlefont{\hfill\Large\bfseries}
\renewcommand\cftaftertoctitle{\hfill\mbox{}}


\usepackage{tocloft}
\renewcommand{\cftpartfont}{\itshape\bfseries}
\renewcommand{\cftchapfont}{\bfseries}


%%% Citing %%%
%\usepackage[natbib=true]{biblatex} 											% Citing
\usepackage[authoryear]{natbib} 												% Citing
%\renewcommand{\bibsection}{}
%\usepackage{usebib}
%\usepackage{keyval}
\setcitestyle{authoryear,aysep={},open={(},close={)}}
%\usepackage{bibentry}
% \makeatletter
% \renewcommand\BR@b@bibitem[2][]{\BR@bibitem[#1]{#2}\BR@c@bibitem{#2}}
% \makeatother
%\nobibliography*



\usepackage[hypertexnames=false,backref=page]{hyperref}															% Define links (color, shape, etc)
\newcommand*{\hyref}[2]{\hyperref[#1]{#2 \ref{#1}}}

\hypersetup{
    pdffitwindow=false,									% Window fit to page when opened
    pdfstartview={XYZ null null 1.00},					% Fits the zoom of the page to 100%
    pdfnewwindow=true, 									% Links in new window
    colorlinks=true,									% false: boxed links; true: colored links
    linkcolor={red!50!black},							% Color of internal links (black is necessary for printing quality)
    citecolor={blue!50!black},							% Color of links to bibliography
    urlcolor=black,										% Color of external links
%	hidelinks, 											% No colour nor borders in links
	linkbordercolor={white},							% Color of links from hyperref; enables dropping of ugly borders in citations
    pdfauthor = {Duarte Goncalves},
    pdfkeywords = {1, 2, 3},
    pdftitle = {},
    pdfsubject = {},
    pdfpagemode = UseNone,
    backref = true,
}
\setlength{\bibsep}{0pt plus 0.3ex} 											% Determines space between entries in bibliography
\bibpunct{(}{)}{;}{a}{,}{,} 													% Citing Type; see natbib reference shee

\addto\extrasenglish{															% Change \autoref automatic labels
\renewcommand{\partautorefname}{Section}
\renewcommand{\chapterautorefname}{Section}
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}
\renewcommand{\figureautorefname}{fig.}
\renewcommand{\tableautorefname}{table}
\renewcommand{\equationautorefname}{eq.}
}

\makeatletter
\DeclareRobustCommand\citepos													% Create possessives with \citepos[e.g.][p. Y]{Key}: e.g. Key's (Year, p. Y)
  {\begingroup\def\NAT@nmfmt##1{{\NAT@up##1's}}%
   \NAT@swafalse\let\NAT@ctype\z@\NAT@partrue
   \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}

\pretocmd{\NAT@citex}{%
  \let\NAT@hyper@\NAT@hyper@citex
  \def\NAT@postnote{#2}%
  \setcounter{NAT@total@cites}{0}%
  \setcounter{NAT@count@cites}{0}%
  \forcsvlist{\stepcounter{NAT@total@cites}\@gobble}{#3}}{}{}
\newcounter{NAT@total@cites}
\newcounter{NAT@count@cites}
\def\NAT@postnote{}


\def\NAT@hyper@citex#1{%														% Include postnote and \citet closing bracket in hyperlink
  \stepcounter{NAT@count@cites}%
  \hyper@natlinkstart{\@citeb\@extra@b@citeb}#1%
  \ifnumequal{\value{NAT@count@cites}}{\value{NAT@total@cites}}
    {\if*\NAT@postnote*\else\NAT@cmt\NAT@postnote\global\def\NAT@postnote{}\fi}{}%
  \ifNAT@swa\else\if\relax\NAT@date\relax
  \else\NAT@@close\global\let\NAT@nm\@empty\fi\fi								% Avoid compact citations
  \hyper@natlinkend}
\renewcommand\hyper@natlinkbreak[2]{#1}


\patchcmd{\NAT@citex}															% Avoid extraneous postnotes, closing brackets
  {\ifNAT@swa\else\if*#2*\else\NAT@cmt#2\fi
   \if\relax\NAT@date\relax\else\NAT@@close\fi\fi}{}{}{}
\patchcmd{\NAT@citex}
  {\if\relax\NAT@date\relax\NAT@def@citea\else\NAT@def@citea@close\fi}
  {\if\relax\NAT@date\relax\NAT@def@citea\else\NAT@def@citea@space\fi}{}{}
\patchcmd{\NAT@cite}{\if*#3*}{\if*\NAT@postnote*}{}{}

\makeatother
\newcommand*{\headerleft}{}
\newcommand*{\headerright}{~}
\newcommand*{\footright}{\thepage}
\newcommand*{\footcenter}{~}
\newcommand*{\footleft}{~}

\newpagestyle{body}{
  \sethead[\ifthenelse{\value{page}=0}{}{\headerleft}][][\ifthenelse{\value{page}=0}{}{\headerright}]{\ifthenelse{\value{page}=0}{}{\headerleft}}{}{\ifthenelse{\value{page}=0}{}{\headerright}}
  \setfoot[\ifthenelse{\value{page}=0}{}{\footleft}][\ifthenelse{\value{page}=0}{}{\footcenter}][\ifthenelse{\value{page}=0}{}{\footright}]
  {\ifthenelse{\value{page}=0}{}{\footleft}}{\ifthenelse{\value{page}=0}{}{\footcenter}}{\ifthenelse{\value{page}=0}{}{\footright}}
}

\pagestyle{body}
\usepackage{usebib}
\setcitestyle{authoryear,aysep={},open={(},close={)}}
\newbibfield{journal}
\newcommand*{\citewtitle}[1]{\citeauthor*{#1} (\citeyear{#1}) \usebibentry{#1}{title}}
\newcommand*{\fullcite}[1]{\citeauthor*{#1} (\citeyear{#1}) \usebibentry{#1}{title}. \textit{\usebibentry{#1}{journal}}}



\newtheorem*{abstract}{Abstract}

\newtheoremstyle{named}{}{}{}{}{\bfseries}{.}{.5em}{\thmnote{#3}}
\theoremstyle{named}
\newtheorem*{namedenv}{namedenv}

\makeatletter
\declaretheoremstyle[
	spaceabove=15pt,
	spacebelow=15pt,
%    headformat={\makebox[0pt][r]{\ }\NAME\, \NUMBER: \NOTE},
    headformat=\NAME\, \NUMBER: \NOTE,
    headpunct={},
    notefont=\bfseries,
%  headfont=\normalfont,%\scshape,
	notebraces={}{},
	bodyfont=\normalfont,
	postheadspace=\newline,
	qed=\qedsymbol
]{mythmstyle}
\makeatother
\declaretheorem[style=mythmstyle, title=Example]{examples}



\setlength{\parskip}{0.5em}
\setlength{\parindent}{0cm}
\setstretch{1.15}

\usepackage{amsthm}
\usepackage{afterpage}

\usepackage{footnote}
\makesavenoteenv{minipage}



\usepackage{etoc}
\renewcommand{\cftsecaftersnum}{.}
\renewcommand{\cftsubsecaftersnum}{.}





\titleformat{\section}[block]													% Block to format
{\normalfont\Large\bfseries}{\thesection.}{14pt}{\Large\bfseries}		% Formating the block
\titlespacing*{\section}{0pt}{*1.3}{*0.2}											% Spacing before and after

\titleformat{\subsection}[block]
{\normalfont\large\bfseries}{\thesubsection.}{13pt}{\large\bfseries}
\titlespacing*{\subsection}{0pt}{*1}{*0}

\titleformat{\subsubsection}[block]
{\normalfont\bfseries}{\thesubsubsection.}{12pt}{\normalsize\bfseries}
\titlespacing*{\subsubsection}{0pt}{*1}{*0.8}


\renewcommand\thesection{\arabic{section}}
\renewcommand\thesubsection{\thesection.\arabic{subsection}}
\renewcommand\thesubsubsection{\thesubsection.\arabic{subsubsection}}
\usepackage{longtable}

\makeatletter
\newcommand*\TOCcompute@numwidths [2]{% #1=empty/"local", #2=minimal indent
	\begingroup
		\def\TOCnumwidthB {0pt}%
		\def\TOCnumwidthC {0pt}%
		\def\TOCnumwidthD {0pt}%
		\def\TOCnumwidthE {0pt}%
		\def\TOCnumwidthF {0pt}%
		\def\TOCnumwidthG {0pt}%
% 		\etocsetstyle{part}{}{}{}{}%
% 		\etocsetstyle{chapter}{}
% 			{\setbox0\hbox{\bfseries\etocthenumber\kern#2}}
% 			{\ifdim\wd0>\TOCnumwidthB\edef\TOCnumwidthB{\the\wd0}\fi}{}%
% 		\etocsetstyle{section}{}
% 			{\setbox0\hbox{\bfseries\etocthenumber\kern#2}}
% 			{\ifdim\wd0>\TOCnumwidthC\edef\TOCnumwidthC{\the\wd0}\fi}{}%
		\etocsetstyle{subsection}{}
			{\setbox0\hbox{\bfseries\etocthenumber\kern#2}}
			{\ifdim\wd0>\TOCnumwidthD\edef\TOCnumwidthD{\the\wd0}\fi}{}%
		\etocsetstyle{subsubsection}{}
			{\setbox0\hbox{\bfseries\etocthenumber\kern#2}}
			{\ifdim\wd0>\TOCnumwidthE\edef\TOCnumwidthE{\the\wd0}\fi}{}%
		\etocsetstyle{paragraph}{}
			{\setbox0\hbox{\bfseries\etocthenumber\kern#2}}
			{\ifdim\wd0>\TOCnumwidthF\edef\TOCnumwidthF{\the\wd0}\fi}{}%
		\etocsetstyle{subparagraph}{}
			{\setbox0\hbox{\bfseries\etocthenumber\kern#2}}
			{\ifdim\wd0>\TOCnumwidthG\edef\TOCnumwidthG{\the\wd0}\fi}{}%
		%
		{\global\let\TOCnumwidthB\TOCnumwidthB
		\global\let\TOCnumwidthB\TOCnumwidthC
		\global\let\TOCnumwidthB\TOCnumwidthD
		\global\let\TOCnumwidthB\TOCnumwidthE
		\global\let\TOCnumwidthB\TOCnumwidthF
		\global\let\TOCnumwidthB\TOCnumwidthG}%
		\etocnopar
% 		\csname #1tableofcontents\endcsname
		\typeout{Next TOCs will use \TOCnumwidthB\space for chapter number width}%
		\typeout{Next TOCs will use \TOCnumwidthC\space for section number width}%
		\typeout{Next TOCs will use \TOCnumwidthD\space for subsection number width}%
		\typeout{Next TOCs will use \TOCnumwidthE\space for subsubsection number width}%
		\typeout{Next TOCs will use \TOCnumwidthF\space for paragraph number width}%
		\typeout{Next TOCs will use \TOCnumwidthG\space for subparagraph number width}%
		\endgroup
	}%
	\newcommand*\TOCcomputenumwidths [1][0.5em]{%
	\TOCcompute@numwidths {}{#1}%
	}%
	\newcommand*\TOCcomputelocalnumwidths [1][-10em]{%
	\TOCcompute@numwidths {local}{#1}%
}%
\makeatother

\makeatletter
\providecommand*{\hrefurl}{\hyper@normalise\hrefurl@}
\providecommand*{\hrefurl@}[2]{\hyper@linkurl{#2}{#1}}
\makeatother


\definecolor{mathematica1}{rgb}{0.368417, 0.506779, 0.709798}
\definecolor{mathematica2}{rgb}{0.880722, 0.611041, 0.142051}
\definecolor{mathematica3}{rgb}{0.560181, 0.691569, 0.194885}
\definecolor{mathematica4}{rgb}{0.922526, 0.385626, 0.209179}
\definecolor{mathematica5}{rgb}{0.528488, 0.470624, 0.701351}

